Secure-by-synthesis network with active deception and temporal logic specifications

This paper is concerned with the synthesis of strategies in network systems with active cyber deception. Active deception in a network employs decoy systems and other defenses to conduct defensive planning against the intrusion of malicious attackers who have been confirmed by sensing systems. In this setting, the defender's objective is to ensure the satisfaction of security properties specified in temporal logic formulas. We formulate the problem of deceptive planning with decoy systems and other defenses as a two-player games with asymmetrical information and Boolean payoffs in temporal logic. We use level-2 hypergame with temporal logic objectives to capture the incomplete/incorrect knowledge of the attacker about the network system as a payoff misperception. The true payoff function is private information of the defender. Then, we extend the solution concepts of $omega$-regular games to analyze the attacker's rational strategy given her incomplete information. By generalizing the solution of level-2 hypergame in the normal form to extensive form, we extend the solutions of games with safe temporal logic objectives to decide whether the defender can ensure security properties to be satisfied with probability one, given any possible strategy that is perceived to be rational by the attacker. Further, we use the solution of games with co-safe (reachability) temporal logic objectives to determine whether the defender can engage the attacker, by directing the attacker to a high-fidelity honeypot. The effectiveness of the proposed synthesis methods is illustrated with synthetic network systems with honeypots.

==> model-attackgame.tex <==

 

\todo[inline]{Investigate software defined network}


\begin{remark}  In this model, the network connectivity is directly incorporated
  into the transition relations.  Though we use the set notation of
  transition relation for notation convenience, the transitions are
  deterministic.
\end{remark}
%\color{blue}
\paragraph*{Extension} In order to capture the capability of an attacker who can carry out attacks in multiple locations simultaneously, we propose to augment the transition system  with the following states and actions:
\begin{itemize}
    \item We will augment the state of the system with a \emph{memory} state: A set of hosts that have been visited by the attacker. For example, given $s_1=(h_1,priv_1,b_1, 0)$--a state of the attacker, we augment a set $X$ to trace the visited host, $\hat s_1=(s_1, X)$. A transition $s_1\xrightarrow{a_1} s_2$ will be changed to $(s_1,X)\xrightarrow{a_1}(s_2, X \cup \{h_2\})$ given that $s_2=(h_2,priv_2,b_2,1)$.
    \item Combinatorial attack actions: To capture the attacks at multiple hosts, we can augment the action space of the attacker by a powerset of hosts. The attacker can select a set from the powerset to carry out simultanuous attacks.
\end{itemize}

The extension does not change the nature of the game transition system but introduces more states and transitions. This can potentially lead to scalability issue. 
\normalcolor


\begin{example}
\label{ex:simplegame_2}
Continue with the example, the set of states P2 believes to be in $\win_2^2$  is $\{(0,0,0), (1,0,0), (2,0,0), (3,1,1), (4,2,1)\}$, computed with $Z_0=\{(3,1,1), (4,2,1)\}$, $Z_1= Z_0\cup \{ (1,0,0), (2,0,0)\}$, and $Z_2= Z_1\cup \{(0,0,0)\}$ and $Z_3=Z_2$. In this example, P2 believes that she has a sure-winning strategy from the initial state. That is, no matter which action P1 takes, P2 can ensure a visit to a target, in her perceptual game. For example, if P1 takes action $a_1$, then P2 can choose freely between $b_1$ and $b_2$ to reach a target given her misperceived labeling function.

Next, let's consider the true winning region of P2  against P1's safety specification $\Always \neg \goals$. $\win_2^1$ is computed again using Alg.~\ref{alg:zielonka} with the set $F= \{(3,1,1)\}$. We have $\win_2^1 =\{(3,1,1), (1,0,0)\}$, computed with $Z_0= \{(3,1,1)\}$, $Z_1=\{1,0,0\}\cup Z_0$, and $Z_2=Z_1$. P1 has a winning safety strategy $\pi_1(0,0,0)=a_2$ to ensure that P2 can stay within the set of safe states. Better, because the only outgoing transition from $(2,0,0)$ is to $(4,2,1)$. P1 can ensure that P2 will visit a honeypot by visiting state  $(4,2,1)$. 


However, if the initial state is not $(0,0,0)$ but $(1,0,0)$, then P2, without any misperception in the labeling function, can ensure to visit a targeted host by taking action $b_1$ to reach state $(3,1,1)$. When P2 misperceives the labeling function, then P2 is possible to take action $b_2$ by mistake (as she perceives the winning region is $\win_2^2$). This mistake by P2 can be used by  P1 to lure P2 into a decoy.
\end{example}

Next, we are interested in the cases when 1) P1 does not have a almost-sure-winning strategy from the initial state of the game; and  2) P2 has misperceived labeling function. We aims to ask the following two question: Is there a  almost-sure winning strategy for P1 with P2's labeling misperception? How to allocate the location of honeypot such that P1 can have an almost-sure winning strategy from the initial state of the game?


==> synthesis-labeling.tex <==

\begin{align}
\label{eq:almost_pre}
\begin{split}
      %  \apre_1(X, Y;\pi_2^\multiset) & = \{v\in V_1 \mid \exists a_1\in A_1 \text{ such that } \Delta(v_1,a_1)\in X.\}\\
        \apre_2(X,Y;\pi_2^\multiset) & = \{v\in V_2\mid \forall a_2\in \pi_2^\multiset(v) \text{ such that } \Delta(v_2,a_2)\in Y \\
        &\text{ and } \exists a_2 \in  \pi_2^\multiset (v_2) \mbox{ such that } \Delta(v_2,a_2)\in X\}
        \end{split}
\end{align}


The set $\apre_2(X,Y;  \pi_2^\multiset)$ outputs a set of states from which P1 can ensure that, no matter which strategy P2 uses from the permissive strategy, the game state will \emph{stay} within the set $Y$. Further, P1 can ensure that no matter which stratey P2 uses, there exists an action, with which P2 will take with a nonzero probability, to reach the set $X$ in one step.

Finally, the almost-sure winning region for P1's safety objective can be computed using Algorithm~\ref{alg:safety} with two inputs, the hypergame transition system $\hyperts$  and a set $B\coloneqq\acc_{S}$ that specifies the winning condition of P1: P1 wins if and only if he can force the game to stay within the set $B$ indefinitely.
    
    

P1's winning strategy is also a multi-strategy:
\[
\pi_1^\multi(v; \acc_{S}) = \{d \in\dist{A_1} \mid \supp(d)\subseteq \win_1(\acc_{S})\}.
\]
That is, P1 chooses actions to ensure the game staying within $\win_1(\acc_{S})$. By construction, $\win^1(\acc_{S}) \subseteq \acc_{S}$, by staying within the set $\acc_{S}$, P1 ensures the game stay within the set $\acc_{S}$.

\paragraph*{Almost-sure deceptive winning for P1's safe-till-reach objective}
P1 prefers to lure P2 into visiting the set $\acc_{R}$. To achieve this objective, P1 also need to ensure the primary goal--staying in the set of safe states $\acc_{S}$--must be fulfilled.

Thus, the almost-sure winning for $(v \in \acc_{S})\until (v\in \acc_{R})$ can be computed using Algorithm~\ref{alg:lure} with three inputs: The hypergame transition system $\hyperts$, the set $B$ of states to stay with probability one, and a set $C$ of states to visit with probability one. Letting $B\coloneqq \acc_{S}$ and $C\coloneqq \acc_{R}$, the algorithm is  understood intuitively as follows: The set $X_i$ over iterations keeps track of a set of states from which P1 can ensure a visit to $\acc_{R}$ with a positive probability, while  staying in the set $Y_j$. Then, if there is a state in $Y_j$ from which P1 cannot force a run to $\acc_{R}$ with a positive probability, then that state should not be visited and considered  \emph{unsafe} for P1. Then, P1 removes that state from $Y_j$ to obtain $Y_{j+1}$. Because the set of ``safe'' states are changed, the fixed point $X$ in the inner iteration should be recomputed with respect to the new set--$Y_{j+1}$. The algorithm stops when the outer iteration finds a fixed point. 
    We denote the fixed point $Y^\ast = \win_1(\acc_{S}, \acc_{R}; \pi_2^\multiset)$.
    



\begin{algorithm}
\caption{\label{alg:lure}  Almost-Sure Winning for P1 given P1's winning condition $B\until C$ (staying in $B$ until reaching $C$) and P2's multiset strategy $\pi_2^\multiset$.}
\begin{algorithmic}[1]
\item[\textbf{Inputs:}] $\left(\hyperts=(V=V_1\cup V_2, A_1\cup A_2, \Delta), (B, C)\right)$. 

    \State  $Y_0\leftarrow B$,  $j\leftarrow0$
\While{True}
    \State $X_0\leftarrow C$, $i\leftarrow0$
    \While{True}
        \State 
        $X_{i+1} \leftarrow  X_i \cup \pre_{1}(X_i;\pi_2^\multiset )\cup \apre_2(X_i, Y_j;\pi_2^\multiset)$ 
        \If {$X_{i+1} = X_i$}
        \State $Y_{j+1}\leftarrow X_i$
            \State End Loop
        \EndIf
        \State $i\leftarrow i+1$
    \EndWhile
    \If {$Y_{j+1}= Y_j$ }
    \State $\win_1(B, C; \pi_2^\multiset) \leftarrow Y$ 
    \State End Loop
    \EndIf
          \State  $j\leftarrow j+1$
    \EndWhile
    \State \Return $\win_1(B, C;\pi_2^\multiset)$
\end{algorithmic}
\end{algorithm}  
    
    
    
    
    \begin{theorem}
    For a game transition system $\hyperts$ and P1's preference over two objectives: $\Always (v \in \acc_{S})$ and $(v\in \acc_{S})\until (v\in \acc_{R})$. Algorithm~1 and Algorithm~2 give two set $\win_1(\acc_{S};\pi_2^\multiset)$ and $\win_1(\acc_{S}, \acc_{R};\pi_2^\multiset)$. \begin{itemize}
        \item For any state $v\in \win_1(\acc_{S}; \pi_2^\multiset)$,  P1 has a memoryless multi-strategy with respect to objective $\Always (v \in \acc_{S} )$.
        \item For any state $v\in \win_1(\acc_{S}, \acc_{R}; \pi_2^\multiset)$, P1 has a memoryless, deterministic strategy with respect to objective $(v\in \acc_{S})\until (v\in \acc_{R}  )$.
        \item The winning region satisfies \[
        \win_1(\acc_{S},\acc_{R};\pi_2^\multiset)\subseteq \win_1(\acc_{S};\pi_2^\multiset).
        \]
    \end{itemize}
\end{theorem}


\begin{example}
Let's use the simple example in Ex.~\ref{ex:simplegame_2} to illustrate the computation of almost-sure winning regions given two objectives: $\Always (v\in \acc_{S})$   and $(v\in \acc_{S})\until (v\in \acc_{R})$. 
In this example, it is reminded that $\pi_2^\multiset(2,0,0)=\{\{b_1\}\}$
 and $\pi_2^\multiset(1,0,0)=\{\{b_1\}, \{b_2\}, \{b_1,b_2\}\}$.
 
Case 1: $\Always (v\in \acc_{S})$. Given the set $\acc_{S}=\{(0,0,0), (1,0,0) ,(2,0,0), (4,2,1)\}$ and $X_0=\acc_{S}$, we have $\pre_1(X_0; \pi_2^\multiset) = \{(0,0,0), (4,2,1)\}$ and $\pre_2(X_0;\pi_2^\multiset) = \{(2,0,0)\}$. Note that at state $(2,0,0)$,  P2 can only select action $b_1$ and reach $(4,2,1)$, which is in $X_0$. 
At state $(1,0,0)$, there exists a set $\{b_1,b_2\}$ in $\pi_2^\multiset(1,0,0)=\{\{b_1\}, \{b_2\}, \{b_1,b_2\}\}$. Action $b_1$ triggers a transition from $(1,0,0)$ to $(3,1,1)$--not in $\acc_{S}$. Thus, state $(1,0,0)$ is not in $\pre_2(X_0;\pi_2^\multiset) $.

The set $X_1=X_0 \cap(\pre_1(X_0; \pi_2^\multiset) \cup   \pre_2(X_0;\pi_2^\multiset) =\{(0,0,0), (4,2,1),  (2,0,0)\}$. $X_2= X_1 \cap(\pre_1(X_1; \pi_2^\multiset) \cup   \pre_2(X_1;\pi_2^\multiset) = \win_1(\acc_{S})$. Because the initial state $(0,0,0)$ is in the set $ \win_1(\acc_{S})$, P1 has a strategy to satisfy his safety objective. 

Case 2: $(v\in \acc_{S})\until (v\in \acc_{R})$. Alg.~\ref{alg:lure} is used to solve P1's almost-sure winning strategy. Given $X_0 =\acc_{R}= \{(4,2,1)\}$ and $Y_0=\acc_{S}$, $\apre_2(X_0,Y_0;\pi_2^\multiset)  =\{(2,0,0)\}$ and $\pre_1(X_0;\pi_2^\multiset) = \emptyset$. We have $X_1 = \{(4,2,1), (2,0,0)\}$. $X_2= X_1\cup \{(0,0,0)\}=X_3$. Letting $Y_1= X_2$. A fixed point is reached in both inner and outer loops and $\win_1(\acc_{R},\acc_{S}; \pi_2^\multiset) = \{(0,0,0), (4,2,1),  (2,0,0)\}$.

In both cases, P1, by selecting action $a_2$ from the initial state, can ensure not only the game state staying the set of safe states but also enforce P2 to visit a decoy, \ie, reaching $(4,2,1)$.


         Next, we make a small change to the game transition function by adding a transition $(2,0,0)\xrightarrow{ b_1} (1,0,0)$, shown in blue in Fig.~\ref{fig:hyperts_ex2}. This new transition introduces changes in P2's multi-strategy $\pi_2^\multiset(2,0,0)=\{\{b_2\}, \{b_1\}, \{b_1,b_2\}\}$. Then, when we solve the almost-sure winning strategy for P1 given his objective $\Always (v\in \acc_{S})$.  $X_1= \{(4,2,1), (2,0,0)\}$, $X_2= \{(4,2,1)\} = \win_1(\acc_{S};\pi_2^\multiset)$, which does not include the initial state. Because $\win_1(\acc_{S},\acc_{R}; \pi_2^\multiset)\subseteq \win_1(\acc_{S};\pi_2^\multiset)$, P1 does not have a winning strategy to achieve any of his objectives from the initial state $(0,0,0)$.
         \end{example}
         
         It is observed that the location of honeypots determines the existence of P1's winning strategy for both safety and deceptive objectives. To this end, we propose to investigate the resource allocation problem: How to allocate $k$ honeypots so that P1 has a winning strategy for specification $\Always (v\in \acc_{S})$ and $(v\in \acc_{S})\until (v\in \acc_{R})$?



\todo[inline]{The following is to be revised.}
\section{Almost-sure safety with one-sided partial observation}


\section{Almost-sure deceptive winning with honeypot allocation}

In this section, we consider the case when P1's losing given the initial state of the game, for its safety and safe-till-reach specifications, respectively. Formally, our problem is stated as follows.
\begin{problem}
Consider the dynamic interaction between two players modeled as a transition system $\game=(S, A_1\cup A_2, T)$, select the location of $k$ hosts to be honeypot such that in the constructed hypergame transition system $
  \hyperts= \langle 
(S\times Q_1\times Q_2), A_1\cup A_2, \Delta, v_0, \acc_{R}, \acc_{S}, \acc_2 \rangle$ 
     P1 has an almost-sure winning strategy in the hypergame given P2's misperception for satisfying 
\begin{itemize}
\item Safety objective:  $\Always (v\in \acc_S)$.
\item Safe-till-reach objective:  $(v\in \acc_{S})\until (v\in \acc_{R})$.
\end{itemize}
\end{problem}

\subsection{Almost-sure deceptive safe allocation of honeypots}

First, it is noted that no matter the choice of honeypot locations, the set of states in $\acc_S$, $\acc_{R}$ and $\acc_{2}$ is that $\acc_{R} = \acc_S\cap \acc_{2}$. 

\begin{lemma} If P1 has a winning strategy in the game given P2's objective $\Eventually (v\in \acc_2)$, then P2 satisfies the safety objective because $\Always \neg (v\in \acc_2) \implies \Always (v\in \acc_S)$.
\end{lemma}

\todo[inline]{make it formal and prove}

The locations of honeypots and critical hosts jointly determine the set $\acc_2$. Determining the allocation of honeypots require  design of P2'S perceptual game and P1's winning strategy.

Consider a game arena with no honeypot host. The  hypergame transition system $\hyperts^0$ can be constructed as 
\[
\hyperts= \langle 
(S\times Q_1\times Q_2), A_1\cup A_2, \Delta, v_0, \acc_R^0 = \emptyset, \acc_{S}^0, \acc_2^0 \rangle.
\]
P2's almost-sure winning policy can be computed as $\pi_2^\multiset$ and winning region is $\win_2^0$
Suppose there are $n$ locations among which P1 can select a subset to be honeypot. 

We augment the action sets of P1 with the choice of determining whether a state should be labeled with decoy. A new game with P1's augmented action set is
\[
(V_1 \cup V_2 , A_1\times A_2 , \hat{\Delta}) 
\]
where the transition function is defined by: Given $(s,q_1,q_2)\xrightarrow{a} (s',q_1',q_2')$.

if $s'$ is a host that can be honeypot.
\[
\hat{\Delta} ((s,q_1,q_2),  (a,\decoys))= (s',q_1',q_2'') 
\] $q_1'' = \delta(q_1, \decoys)$.
\[
\hat{\Delta} ((s,q_1,q_2),  (a,\emptyset)= (s',q_1',q_2') 
\] $q_1' = \delta(q_1, \emptyset)$.

if $s'$ is a host that cannot be a honeypot.
\[
\hat{\Delta} ((s,q_1,q_2),  (a,\emptyset)= (s',q_1',q_2') 
\] $q_1' = \delta(q_1, \emptyset)$.

After this construction, define the set $\acc_R = \{(s,q_1,q_2) \mid q_1 \in F_r\}$.

In this newly constructed game, P1 is to ensure the existence of a winning strategy for $\acc_S\until \acc_R$ given P2's multi-set strategy $\pi_2^\multiset$.  now the decision has included the location of honeypots. 

  
In addition, P1 only needs to guard against P2's move into reaching a critical host. We can prove the following claim:

Claim: Given $\acc_2  = \acc_C\cup \acc_R$. If P1 has a sure-winning strategy given P2's multi-set policy $\pi_2^\multiset$ with respect to objective $\Eventually \acc_C$. Then this strategy is winning given P2's multi-set strategy with respect to $\Eventually (\acc_C\cup \acc_R)$.

proof:  if P2 pursues $\Eventually \acc_C\lor \Eventually \acc_R$ and P1 can ensure P2 does not satisfy $\Eventually \acc_C$, then P2 can only satisfy $\Eventually \acc_R$--running into P1's decoys. 
 
\begin{comment}

We consider a special case of the level-2 hypergame: When P1
manipulates P2's perception of the labeling function, the effect of
this manipulation is reflected in addition and deletions of
transitions in P2's perceptual task automaton.


  Next, we construct the game $\game_2$ using the product of game
  arena $G$ and automaton $\calA^2$. The sure winning policy $\mu$ for
  P2 can be computed from $\game_2$ using solutions of turn-based
  games.

    With the knowledge of the sure-win policy
    $\mu: S\times Q\rightarrow 2^{A_2}$, the following algorithms
    makes a joint decision for labeling manipulation and actions for
    safety objective: P1 is to ensure a set $S\times U \times Q$ is
    not visited by P2, given P2 following her sure-win policy
    $\mu$. We consider two cases of labeling manipulation:

    \paragraph*{Case I: Arbitrarily changing the labeling function}

    Assuming that P1 can change the mask function.  Let $\Theta$ be
    all possible evaluations of $\theta$ in the mask function.

    \begin{itemize}
    \item let the initial set $X_0 = S\times F_1\times Q$. Initialize
      $\gamma: X_0\rightarrow 2^\Theta$ as $\gamma(s,q_1,q_2) =\Theta$
      for any $(s,q_1,q_2)\in X_0$. Let $i=0$.
    \item For any state $(s,q_1,q_2) \in X_i$, compute the following set
      \begin{multline*}
        \mbox{Post}(s,q_1,q_2)= \{ (s',q'_1,q_2')\mid \exists (a,
        \theta) \in A_1\times \gamma(s,q_1,q_2), \forall b\in
        \mu(s,q_2), \\
        T((s,q_1,q_2), (a,b)) = (s',q_1',q_2') \in X_0 \land q_2' =
        \delta_2(q_2, \mask(L(s', \theta)) \} \}
      \end{multline*}
      If $\mbox{Post}(s,q_1,q_2)\ne \emptyset$, then let
      \begin{multline*}
        \pi(s,q_1,q_2) = \{(a,\theta)\mid \forall b\in \mu(s,q_2),\\
        T((s,q_1,q_2), (a,b)) = (s',q_1',q_2')\land q_2' =
        \delta_2(q_2, \mask(L(s', \theta)) \}.
      \end{multline*}
      and let $\gamma(s,q_1,q_2)= \Pi_{\Theta}( \pi(s,q_1,q_2))$ where
      $\Pi_2$ is the projection operator which extracts the second
      component from the policy $\pi(s,q_1,q_2)$.
    \item Let
      $X_{i+1} = X_i - \{(s,q_1,q_2) \mid
      \mbox{Post}(s,q_1,q_2)=\emptyset \}$.  If $X_{i+1}=X_i$, then
      output $X= X_{i+1}=X_i$. Otherwise, then let $i\rightarrow i+1$
      and return to step 2.
      \end{itemize}


      However, the sure-win region computed above assumes no
      constraint on how P1 can switch between different labeling
      functions. It is not feasible in some situation. For example, in
      static decoy allocation, P1 has to choose one $\theta$ (where to
      place the decoys) and cannot change $\theta$ online after this
      decision.

      \paragraph*{Case II: Restricted switching}

      We show that a second pruning step can be performed based on the
      subgraph induced by $(\pi, \mu)$ to incorporate constraints in
      switching between games.

      Let $\eta: \Theta \rightarrow 2^\Theta$ that maps a current
      $\theta$ to a subset of $\Theta$ one can switch to. A special
      case is $\eta(\theta)=\theta$ a one-to-one mapping, reflecting
      the case when P1 cannot change $\theta$ online.

      The second step is described as follows: 1) First, we eliminate
      the following transitions in the subgraph induced by
      $(\pi, \mu)$. For an action $a\in A_1$, a transition
      \[
        (s,q_1,q_2)\xrightarrow{a} (s',q'_1,q'_2)
      \]
      is eliminated if
      $\gamma(s',q'_1,q'_2) \cap \eta(\gamma(s,q_1,q_2)) = \emptyset
      $. That is, the set of switchings required at state
      $(s',q'_1,q'_2) $ is not feasible given the set of possible mask
      parameters at the state $(s,q_1,q_2)$. After this elimination,
      we can proceed to recompute the winning region. The computation is only needed once.

      \todo[inline]{may be there is a way to combine two as one.}
      

      
      \newpage
      




Given the additional capability that P2 can transit to any state which
has been previously visited, we construct the following hypergame,
with modifications in the state space and the transition function of
the hypergame in Def.~\ref{def:hypergameTS}.


First, we define a function to characterize the capability of P2
transiting to a previously visited state.  Let
$\Gamma: S\rightarrow 2^S$ be a function such that if P2 visited
$s\in S$ in the past, then she can initiate a transition to any state
in the set $\Gamma(s)$ in the future. The function $\Gamma$ can be
recursively generalized to sets.
$\Gamma(X \cup\{s\}) = \Gamma(X) \cup \Gamma(s)$ where $X\subseteq S$.
\begin{definition}
  \label{hypergame}
  Given two task automaton $\calA^1 = (Q, \Sigma, \delta_1, q_0, F_1)$
  and $\calA^2 = (Q, \Sigma, \delta_2, q_0, F_2)$.  let
  $L_1: S\rightarrow 2^\calAP$ be the labeling function of P1 and
  $L_2: S\rightarrow 2^\calAP$ be the labeling function perceived by
  P2.  Given the function $\Gamma$, a hypergame transition system is a
  tuple
  \[
  \langle 
(S\times Q\times Q), A_1\cup A_2, \Delta, \acc_1, \acc_2 \rangle
\]
where
\begin{itemize}
\item $V= S\times Q\times Q \times 2^S$ is a set of states. A state
  $v= (s,q_1,q_2, X)$ includes the state $s$ of the game arena, P1
  perceived task state $q_1$, P2 perceived task state $q_2$, and a set
  $X$ of states that P2 can transit to.
\item $A_1\cup A_2$ is a set of actions and $\jump$ is a unique action of P2.
\item
  $\Delta: V \times (A_1\cup A_2)\rightarrow 2^V$ is the transition function, defined by
  \begin{itemize}
    \item $v= (s,q_1,q_2,X)$, P1 or P2 uses $a\in A_1\cup A_2$ and triggers a deterministic transition:
  \[
    \Delta((s,q_1,q_2,X),a)=  (s', q_1',q_2', X \cup \Gamma(s')) 
  \]
  where $s' = T(s, a)$, $q_1' = \delta_1(q_1, L_1(s'))$, and $q_2' = \delta_2(q_2, L_2(s'))$.
  \item $v=  (s,q_1,q_2,X)$, P2 applies $\jump$ to trigger a nondeterministic transition:
  \[
    (s', q_1',q_2', X)\in   \Delta((s,q_1,q_2,X),\jump) 
  \]
  if $s' \in X$, $q_1' = \delta(q_1, L_1(s'))$, and
  $q_2' = \delta(q_2, L_2(s'))$.
  \end{itemize}
\item $\acc_1 = S\times F_1 \times Q \times 2^V $ specifies the
  objective of P1. 
\item $\acc_2 = S\times Q \times F_2 \times 2^V $ specifies the
  objective of P2.
\end{itemize}
\end{definition}
\end{comment}

